Isabelle technology for the Archive of Formal Proofs with application to MMT

This is an overview of the Isabelle technology behind the Archive of Formal Proofs (AFP). Interactive development and quasi-interactive build jobs impose significant demands of scalability on the logic (usually Isabelle/HOL), on Isabelle/ML for mathematical tool implementation, and on Isabelle/Scala for physical system integration --- all integrated in Isabelle/PIDE (the Prover IDE). Continuous growth of AFP has demanded continuous improvements of Isabelle performance. This is a report on the situation in Isabelle2019 (June 2019), with notable add-ons like prover session exports and headless PIDE for automated updates based on semantic information. An example application is Isabelle/MMT, which is able to turn all of Isabelle + AFP into OMDoc and RDF triples, but it is straight-forward to reuse the Isabelle technology for other applications.

==> session.tex <==
\input{Paper.tex}


